Beyond Intrinsic Motivation: The Role of Autonomous Motivation in User Experience

Motivation and autonomy are fundamental concepts in Human-Computer Interaction (HCI), yet in User Experience (UX) research they have remained surprisingly peripheral. We draw on Self-Determination Theory (SDT) to analyse autonomous and non-autonomous patterns of motivation in 497 interaction experiences. Using latent profile analysis, we identify 5 distinct patterns of motivation in technology use -- "motivational profiles" -- associated with significant differences in need satisfaction, affect, and usability. Users' descriptions of these experiences also reveal qualitative differences between profiles: from intentional, purposive engagement, to compulsive use which users themselves consider unhealthy. Our results complicate exclusively positive notions of intrinsic motivation, and clarify how extrinsic motivation can contribute to positive UX. Based on these findings we identify open questions for UX and SDT, addressing "hedonic amotivation" -- negative experiences in activities which are intrinsically motivated but not otherwise valued -- and "design for internalisation" -- scaffolding healthy and sustainable patterns of engagement over time.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography


Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeTeX

==> old_results.tex <==


\db{START OF OLD MOTIVATIONAL PROFILES COMPARISON}
\subsection{Characteristics of the Motivational Profiles} \label{sec:profile_descriptions_old}
Next, we highlight features of the five profiles identified via latent profile analysis. %, with regards to UX ratings and the free text analysis. 
For each profile we describe the pattern of motivational regulations which characterises the profile, the technologies selected by participants, and the distributions of scores on the quantitative UX measures. %hypothesis and non-hypothesis variables. 
We also describe the results of the free text analysis for each profile, to shed additional light on the contextual and experiential factors which characterised each profile's engagement with the technology. 
A full breakdown of technologies per profile is found in \autoref{tab:profile_technologies}.
Motivational regulation scores for each profile are depicted in \autoref{lpa_profiles}, with descriptive statistics 
reported in \autoref{tab:umi_descriptive} (\autoref{appA}). %Outcome values for hypothesis variables 
Descriptive statistics for need satisfaction and other UX ratings are listed in \autoref{tab:bns_var} and \autoref{tab:other_hyp_var}, respectively. %ratings are plotted in \autoref{bch_hyp_plot}, with descriptive statistics reported in \autoref{tab:bns_var}. Other UX ratings are depicted in \autoref{bch_expl_plot}, with descriptive statistics in \autoref{tab:other_hyp_var}. Full data and analysis code is shared at \url{https://osf.io/eny6v/?view_only=422a3f32b1804cdab98cb0c12e0bf3ac}


 \begin{figure}s
  \includesvg[inkscapelatex=false,width=1\linewidth]{lpa_profiles.svg}  
  \vspace{-2em}
  \caption{The five profiles identified by latent profile analysis.  Higher scores on constructs to the left indicate a less autonomous motivational profile, and higher scores on constructs to the right indicate a more autonomous profile. The black points indicate the mean, error bars show standard errors, boxes show standard deviations. Profile membership in LPA is probabilistic, and membership probability is indicated here by opacity.  am = amotivated, ex = external regulation, ij = introjected regulation, id = identified regulation, it = integrated regulation, im = intrinsic motivation. %Individual regulations are qualitatively different but related. 
}
  \label{lpa_profiles}
 \end{figure}

% ----------------------------------------------------------
%  Outcome variables per Profile table ------------------------------
 
\begin{table}

\caption{\label{tab:bns_var}Basic Need Satisfaction variables per profile. M = mean, CI = confidence interval (lower, upper), SD = standard deviation.}
\vspace{-1em}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{9em}rrccccccccc}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{Autonomy} & \multicolumn{3}{c}{Competence} & \multicolumn{3}{c}{Relatedness} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9} \cmidrule(l{3pt}r{3pt}){10-12}
 & Participants & \% Positive & M & CI & SD & M & CI & SD & M & CI & SD\\
\midrule
\textbf{\cellcolor{gray!6}{Mean Positive}} & \cellcolor{gray!6}{254 (51\%)} & \cellcolor{gray!6}{100.0} & \cellcolor{gray!6}{4.75} & \cellcolor{gray!6}{{}[4.59, 4.91]} & \cellcolor{gray!6}{1.32} & \cellcolor{gray!6}{4.31} & \cellcolor{gray!6}{{}[4.1, 4.53]} & \cellcolor{gray!6}{1.73} & \cellcolor{gray!6}{3.61} & \cellcolor{gray!6}{{}[3.38, 3.84]} & \cellcolor{gray!6}{1.85}\\
\textbf{Mean Negative} & 243 (49\%) & 0.0 & 3.38 & {}[3.19, 3.58] & 1.53 & 3.25 & {}[3.04, 3.46] & 1.64 & 2.93 & {}[2.71, 3.15] & 1.74\\
\midrule
\textbf{\cellcolor{gray!6}{High Quality}} & \cellcolor{gray!6}{165 (33.2\%)} & \cellcolor{gray!6}{74.5} & \cellcolor{gray!6}{5.47} & \cellcolor{gray!6}{{}[5.34, 5.6]} & \cellcolor{gray!6}{0.87} & \cellcolor{gray!6}{5.07} & \cellcolor{gray!6}{{}[4.86, 5.28]} & \cellcolor{gray!6}{1.36} & \cellcolor{gray!6}{4.09} & \cellcolor{gray!6}{{}[3.82, 4.35]} & \cellcolor{gray!6}{1.74}\\
\textbf{Medium} & 146 (29.4\%) & 76.0 & 3.98 & {}[3.79, 4.18] & 1.21 & 3.54 & {}[3.28, 3.81] & 1.65 & 2.97 & {}[2.69, 3.25] & 1.74\\
\textbf{\cellcolor{gray!6}{External}} & \cellcolor{gray!6}{58 (11.7\%)} & \cellcolor{gray!6}{19.0} & \cellcolor{gray!6}{3.26} & \cellcolor{gray!6}{{}[2.85, 3.66]} & \cellcolor{gray!6}{1.57} & \cellcolor{gray!6}{3.86} & \cellcolor{gray!6}{{}[3.47, 4.25]} & \cellcolor{gray!6}{1.50} & \cellcolor{gray!6}{3.80} & \cellcolor{gray!6}{{}[3.28, 4.32]} & \cellcolor{gray!6}{1.99}\\
\textbf{Amotivated I.M.} & 71 (14.3\%) & 9.9 & 3.07 & {}[2.78, 3.35] & 1.23 & 2.08 & {}[1.86, 2.3] & 0.94 & 2.72 & {}[2.39, 3.05] & 1.42\\
\textbf{\cellcolor{gray!6}{Amotivated}} & \cellcolor{gray!6}{57 (11.5\%)} & \cellcolor{gray!6}{3.5} & \cellcolor{gray!6}{2.34} & \cellcolor{gray!6}{{}[2.09, 2.59]} & \cellcolor{gray!6}{0.95} & \cellcolor{gray!6}{2.79} & \cellcolor{gray!6}{{}[2.43, 3.15]} & \cellcolor{gray!6}{1.36} & \cellcolor{gray!6}{1.84} & \cellcolor{gray!6}{{}[1.54, 2.14]} & \cellcolor{gray!6}{1.13}\\
\bottomrule
\end{tabular}}
\end{table}

% \begin{table}
% \caption{\label{tab:bns_var}Basic Needs Satisfaction variables per profile \dtb{fix percentages}. M = mean, SD = standard deviation, CI = confidence interval (lower, upper).}
% \centering
% \resizebox{\linewidth}{!}{
% \begin{tabular}[t]{>{\raggedright\arraybackslash}p{9em}rrcccccccccccc}
% \toprule
% \multicolumn{3}{c}{ } & \multicolumn{3}{c}{Autonomy} & \multicolumn{3}{c}{Competence} & \multicolumn{3}{c}{Relatedness} & \multicolumn{3}{c}{Total Basic Needs} \\
% \cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9} \cmidrule(l{3pt}r{3pt}){10-12} \cmidrule(l{3pt}r{3pt}){13-15}
%  & Participants & \% Positive & M & CI & SD & M & CI & SD & M & CI & SD & M & CI & SD\\
% \midrule
% \textbf{\cellcolor{gray!6}{Mean Positive}} & \cellcolor{gray!6}{254 (51\%)} & \cellcolor{gray!6}{100.0} & \cellcolor{gray!6}{4.75} & \cellcolor{gray!6}{{}[4.67, 4.83]} & \cellcolor{gray!6}{1.32} & \cellcolor{gray!6}{4.31} & \cellcolor{gray!6}{{}[4.21, 4.42]} & \cellcolor{gray!6}{1.73} & \cellcolor{gray!6}{3.61} & \cellcolor{gray!6}{{}[3.5, 3.72]} & \cellcolor{gray!6}{1.85} & \cellcolor{gray!6}{4.23} & \cellcolor{gray!6}{{}[4.15, 4.3]} & \cellcolor{gray!6}{1.20}\\
% \textbf{Mean Negative} & 243 (49\%) & 0.0 & 3.38 & {}[3.29, 3.48] & 1.53 & 3.25 & {}[3.15, 3.35] & 1.64 & 2.93 & {}[2.82, 3.03] & 1.74 & 3.19 & {}[3.11, 3.26] & 1.27\\
% \midrule
% \textbf{\cellcolor{gray!6}{High Quality}} & \cellcolor{gray!6}{165 (165\%)} & \cellcolor{gray!6}{74.5} & \cellcolor{gray!6}{5.47} & \cellcolor{gray!6}{{}[5.34, 5.6]} & \cellcolor{gray!6}{0.87} & \cellcolor{gray!6}{5.07} & \cellcolor{gray!6}{{}[4.86, 5.28]} & \cellcolor{gray!6}{1.36} & \cellcolor{gray!6}{4.09} & \cellcolor{gray!6}{{}[3.82, 4.35]} & \cellcolor{gray!6}{1.74} & \cellcolor{gray!6}{4.88} & \cellcolor{gray!6}{{}[4.81, 4.94]} & \cellcolor{gray!6}{0.89}\\
% \textbf{Medium} & 146 (146\%) & 76.0 & 3.98 & {}[3.79, 4.18] & 1.21 & 3.54 & {}[3.28, 3.81] & 1.65 & 2.97 & {}[2.69, 3.25] & 1.74 & 3.50 & {}[3.42, 3.57] & 0.95\\
% \textbf{\cellcolor{gray!6}{External}} & \cellcolor{gray!6}{58 (58\%)} & \cellcolor{gray!6}{19.0} & \cellcolor{gray!6}{3.26} & \cellcolor{gray!6}{{}[2.85, 3.66]} & \cellcolor{gray!6}{1.57} & \cellcolor{gray!6}{3.86} & \cellcolor{gray!6}{{}[3.47, 4.25]} & \cellcolor{gray!6}{1.50} & \cellcolor{gray!6}{3.80} & \cellcolor{gray!6}{{}[3.28, 4.32]} & \cellcolor{gray!6}{1.99} & \cellcolor{gray!6}{3.64} & \cellcolor{gray!6}{{}[3.47, 3.8]} & \cellcolor{gray!6}{1.30}\\
% \textbf{Amotivated I.M.} & 71 (71\%) & 9.9 & 3.07 & {}[2.78, 3.35] & 1.23 & 2.08 & {}[1.86, 2.3] & 0.94 & 2.72 & {}[2.39, 3.05] & 1.42 & 2.62 & {}[2.52, 2.72] & 0.88\\
% \textbf{\cellcolor{gray!6}{Amotivated}} & \cellcolor{gray!6}{57 (57\%)} & \cellcolor{gray!6}{3.5} & \cellcolor{gray!6}{2.34} & \cellcolor{gray!6}{{}[2.09, 2.59]} & \cellcolor{gray!6}{0.95} & \cellcolor{gray!6}{2.79} & \cellcolor{gray!6}{{}[2.43, 3.15]} & \cellcolor{gray!6}{1.36} & \cellcolor{gray!6}{1.84} & \cellcolor{gray!6}{{}[1.54, 2.14]} & \cellcolor{gray!6}{1.13} & \cellcolor{gray!6}{2.32} & \cellcolor{gray!6}{{}[2.2, 2.45]} & \cellcolor{gray!6}{0.97}\\
% \bottomrule
% \end{tabular}}
% \end{table}



\begin{table}

\caption{\label{tab:other_hyp_var}Other hypothesis variables, per profile. M = mean, SD = standard deviation, CI = confidence interval (lower, upper).}
\vspace{-1em}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{>{\raggedright\arraybackslash}p{9em}rrccccccccc}
\toprule
\multicolumn{3}{c}{ } & \multicolumn{3}{c}{PANAS} & \multicolumn{3}{c}{UMUX} & \multicolumn{3}{c}{Self-Attribution} \\
\cmidrule(l{3pt}r{3pt}){4-6} \cmidrule(l{3pt}r{3pt}){7-9} \cmidrule(l{3pt}r{3pt}){10-12}
 & Participants & \% Positive & M & CI & SD & M & CI & SD & M & CI & SD\\
\midrule
\textbf{\cellcolor{gray!6}{Mean Positive}} & \cellcolor{gray!6}{254 (51\%)} & \cellcolor{gray!6}{100.0} & \cellcolor{gray!6}{1.96} & \cellcolor{gray!6}{{}[1.86, 2.07]} & \cellcolor{gray!6}{0.85} & \cellcolor{gray!6}{6.19} & \cellcolor{gray!6}{{}[6.09, 6.29]} & \cellcolor{gray!6}{0.81} & \cellcolor{gray!6}{5.66} & \cellcolor{gray!6}{{}[5.48, 5.84]} & \cellcolor{gray!6}{1.45}\\
\textbf{Mean Negative} & 243 (49\%) & 0.0 & 0.61 & {}[0.47, 0.74] & 1.08 & 4.54 & {}[4.34, 4.73] & 1.55 & 5.13 & {}[4.91, 5.35] & 1.73\\
\midrule
\textbf{\cellcolor{gray!6}{High Quality}} & \cellcolor{gray!6}{165 (33.2\%)} & \cellcolor{gray!6}{74.5} & \cellcolor{gray!6}{2.35} & \cellcolor{gray!6}{{}[2.24, 2.46]} & \cellcolor{gray!6}{0.72} & \cellcolor{gray!6}{6.01} & \cellcolor{gray!6}{{}[5.85, 6.17]} & \cellcolor{gray!6}{1.07} & \cellcolor{gray!6}{5.88} & \cellcolor{gray!6}{{}[5.71, 6.05]} & \cellcolor{gray!6}{1.11}\\
\textbf{Medium} & 146 (29.4\%) & 76.0 & 1.55 & {}[1.45, 1.66] & 0.65 & 5.97 & {}[5.81, 6.13] & 0.99 & 5.29 & {}[4.99, 5.58] & 1.82\\
\textbf{\cellcolor{gray!6}{External}} & \cellcolor{gray!6}{58 (11.7\%)} & \cellcolor{gray!6}{19.0} & \cellcolor{gray!6}{0.36} & \cellcolor{gray!6}{{}[0.07, 0.64]} & \cellcolor{gray!6}{1.08} & \cellcolor{gray!6}{4.03} & \cellcolor{gray!6}{{}[3.62, 4.45]} & \cellcolor{gray!6}{1.60} & \cellcolor{gray!6}{5.23} & \cellcolor{gray!6}{{}[4.79, 5.66]} & \cellcolor{gray!6}{1.68}\\
\textbf{Amotivated I.M.} & 71 (14.3\%) & 9.9 & 0.21 & {}[0.07, 0.36] & 0.62 & 5.52 & {}[5.31, 5.74] & 0.94 & 5.57 & {}[5.24, 5.9] & 1.43\\
\textbf{\cellcolor{gray!6}{Amotivated}} & \cellcolor{gray!6}{57 (11.5\%)} & \cellcolor{gray!6}{3.5} & \cellcolor{gray!6}{-0.14} & \cellcolor{gray!6}{{}[-0.22, -0.05]} & \cellcolor{gray!6}{0.32} & \cellcolor{gray!6}{3.15} & \cellcolor{gray!6}{{}[2.9, 3.39]} & \cellcolor{gray!6}{0.94} & \cellcolor{gray!6}{4.23} & \cellcolor{gray!6}{{}[3.76, 4.7]} & \cellcolor{gray!6}{1.79}\\
\bottomrule
\end{tabular}}
\end{table}

% ----------------------------------------------------------
%  TECHNOLOGIES PROFILE TABLE ------------------------------
\begin{table}

\caption{\label{tab:profile_technologies}Technology categories per profile and condition, shown as percentage of participants per category, with counts in brackets.}
\vspace{-1em}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}[t]{>{}l|r>{}r|rrrr>{}r|r}
\toprule
Technology Category & Positive & Negative & High 
Quality & Medium & External & Amotivated
 IM & Amotivated & Total\\
\midrule
\cellcolor{gray!6}{social media} & \cellcolor{gray!6}{26\% (67)} & \cellcolor{gray!6}{36\% (87)} & \cellcolor{gray!6}{25\% (41)} & \cellcolor{gray!6}{25\% (36)} & \cellcolor{gray!6}{21\% (12)} & \cellcolor{gray!6}{73\% (52)} & \cellcolor{gray!6}{23\% (13)} & \cellcolor{gray!6}{154}\\
streaming media & 12\% (30) & 6\% (14) & 8\% (13) & 18\% (26) & 0\% (0) & 6\% (4) & 2\% (1) & 44\\
\cellcolor{gray!6}{messaging and Email} & \cellcolor{gray!6}{7\% (17)} & \cellcolor{gray!6}{7\% (17)} & \cellcolor{gray!6}{7\% (11)} & \cellcolor{gray!6}{5\% (8)} & \cellcolor{gray!6}{17\% (10)} & \cellcolor{gray!6}{3\% (2)} & \cellcolor{gray!6}{5\% (3)} & \cellcolor{gray!6}{34}\\
creativity, media, writing & 9\% (22) & 4\% (10) & 8\% (13) & 8\% (11) & 5\% (3) & 1\% (1) & 7\% (4) & 32\\
\cellcolor{gray!6}{computers, phones, tablets} & \cellcolor{gray!6}{5\% (12)} & \cellcolor{gray!6}{4\% (9)} & \cellcolor{gray!6}{5\% (9)} & \cellcolor{gray!6}{5\% (8)} & \cellcolor{gray!6}{3\% (2)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{4\% (2)} & \cellcolor{gray!6}{21}\\
voice assistants & 4\% (10) & 5\% (11) & 4\% (6) & 6\% (9) & 0\% (0) & 1\% (1) & 9\% (5) & 21\\
\cellcolor{gray!6}{finance} & \cellcolor{gray!6}{5\% (12)} & \cellcolor{gray!6}{3\% (8)} & \cellcolor{gray!6}{5\% (8)} & \cellcolor{gray!6}{5\% (7)} & \cellcolor{gray!6}{3\% (2)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{5\% (3)} & \cellcolor{gray!6}{20}\\
workplace technologies & 2\% (6) & 6\% (14) & 2\% (4) & 1\% (2) & 22\% (13) & 0\% (0) & 2\% (1) & 20\\
\cellcolor{gray!6}{gaming} & \cellcolor{gray!6}{4\% (11)} & \cellcolor{gray!6}{3\% (8)} & \cellcolor{gray!6}{2\% (4)} & \cellcolor{gray!6}{5\% (8)} & \cellcolor{gray!6}{3\% (2)} & \cellcolor{gray!6}{7\% (5)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{19}\\
fitness, health and wellbeing & 5\% (12) & 2\% (4) & 8\% (13) & 1\% (1) & 0\% (0) & 0\% (0) & 4\% (2) & 16\\
\cellcolor{gray!6}{AI Chatbots} & \cellcolor{gray!6}{3\% (8)} & \cellcolor{gray!6}{2\% (6)} & \cellcolor{gray!6}{4\% (6)} & \cellcolor{gray!6}{3\% (4)} & \cellcolor{gray!6}{3\% (2)} & \cellcolor{gray!6}{1\% (1)} & \cellcolor{gray!6}{2\% (1)} & \cellcolor{gray!6}{14}\\
information and maps & 4\% (9) & 2\% (4) & 3\% (5) & 4\% (6) & 3\% (2) & 0\% (0) & 0\% (0) & 13\\
\cellcolor{gray!6}{other} & \cellcolor{gray!6}{2\% (4)} & \cellcolor{gray!6}{3\% (8)} & \cellcolor{gray!6}{2\% (3)} & \cellcolor{gray!6}{1\% (2)} & \cellcolor{gray!6}{5\% (3)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{7\% (4)} & \cellcolor{gray!6}{12}\\
shopping & 1\% (2) & 4\% (10) & 1\% (1) & 3\% (5) & 0\% (0) & 1\% (1) & 9\% (5) & 12\\
\cellcolor{gray!6}{learning and education} & \cellcolor{gray!6}{3\% (7)} & \cellcolor{gray!6}{2\% (4)} & \cellcolor{gray!6}{4\% (7)} & \cellcolor{gray!6}{1\% (2)} & \cellcolor{gray!6}{2\% (1)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{2\% (1)} & \cellcolor{gray!6}{11}\\
other entertainment & 1\% (3) & 3\% (8) & 1\% (2) & 1\% (2) & 2\% (1) & 4\% (3) & 5\% (3) & 11\\
\cellcolor{gray!6}{other hardware} & \cellcolor{gray!6}{1\% (3)} & \cellcolor{gray!6}{2\% (4)} & \cellcolor{gray!6}{2\% (3)} & \cellcolor{gray!6}{1\% (2)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{4\% (2)} & \cellcolor{gray!6}{7}\\
software development and analysis & 2\% (4) & 1\% (2) & 2\% (3) & 1\% (2) & 2\% (1) & 0\% (0) & 0\% (0) & 6\\
\cellcolor{gray!6}{browsers} & \cellcolor{gray!6}{1\% (3)} & \cellcolor{gray!6}{1\% (2)} & \cellcolor{gray!6}{1\% (2)} & \cellcolor{gray!6}{1\% (2)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{1\% (1)} & \cellcolor{gray!6}{0\% (0)} & \cellcolor{gray!6}{5}\\
operating system & 1\% (3) & 1\% (2) & 1\% (2) & 1\% (1) & 2\% (1) & 0\% (0) & 2\% (1) & 5\\
\bottomrule
\end{tabular}}
\end{table}

%  Table Ends
%  ---------------------------------------------------------

\begin{figure}[ht]
\includesvg[inkscapelatex=false,width=1\linewidth]{bch_hyp.svg}  
\vspace{-2em}
  \caption{Results for the six variables pre-registered for hypothesis testing. Black points indicate means, error bars show standard error, boxes show standard deviation. Green and red lines indicate indicates means for positive and negative' conditions respectively. Asterisks indicate Holm-Bonferroni adjusted p-values: *** $< 0.001$, ** $< 0.01$, * $< 0.05$.   See \autoref{lpa_profiles} for more details supporting interpretation of the chart. Full tables of results, and plots for non-hypothesis variables are provided in \autoref{appA}}
  \label{bch_hyp_plot}
 \end{figure}

 \begin{figure}[ht]
  \includesvg[inkscapelatex=false,width=1\linewidth]{bch_expl.svg}  
  \vspace{-2em}
  \caption{Results for the non-hypothesis variables. Black points indicate means, error bars show standard error, boxes show standard deviation. Green and red lines indicate indicates means for positive and negative conditions respectively.   See \ref{lpa_profiles} for more details supporting interpretation of the chart. }
  \label{bch_expl_plot}
 \end{figure}



\subsubsection{High Quality}
% High level categorical stuff

% UMI scores
\paragraph{Participants and Technologies}
The High Quality profile was the biggest profile in our sample (n = 165), with the majority of participants (n = 123, 74.5\%) in the positive condition.
Among the chosen technologies, 25\% of accounts addressed
social media, 8\% streaming media, followed by a range of other technologies across workplace technologies, creativity, fitness, and messaging (see \autoref{tab:profile_technologies}).

\paragraph{Motivational regulations}
Of all the profiles, the High Quality profile exhibited the most pronounced skew towards autonomous motivations, with integrated regulation --- the most autonomous form of extrinsic motivation --- most prominent. %, associated with reflectively valued behaviours which are congruent with values and goals. 
Scores for intrinsic motivation and identified regulations are also high, indicating that %aside from deeper meaning and investment, these users
respondents generally found the technology use both inherently satisfying and worthwhile.
At the same time, introjection scores were relatively high: the second highest for any profile, indicating that rigid internal controls also played some role in this profile's motivation to use the technology.
External motivation %(reflecting motivation by expected reward or avoidance of negative outcome) 
was relatively low, but comparable to most other profiles.
Finally, %amotivated regulation 
amotivation was low compared to all other profiles, indicating that the technology use in this profile tended to be more than usually intentional.

%\paragraph{Needs Satisfaction}
\paragraph{UX ratings}
% External variables
The High Quality profile reported the highest levels of need satisfaction, %of any group: 
both across each of the three basic needs (autonomy: M  = 5.47, competence: M  = 5.07, and relatedness: M  = 4.09) as well as the five additional needs. All means were %above 4 (on a scale of 1-7), and 
considerably above the mean need satisfaction ratings
for the positive condition overall. %This is true despite roughly 25\% of participants in this group coming from the negative condition. 
%For most needs this was also the \textit{only} group where mean satisfaction was higher than for the positive condition overall.
Autonomy, self-actualisation-meaning (M  = 4.37), and self-esteem (M  = 5.17) were particularly high relative to other profiles.

%\paragraph{Other Outcome Variables}
The mean PANAS score was 2.35 (on a scale of -5 to 5), indicating positive affect: high compared to all other profiles, and above the mean for the positive condition (M  = 1.96). Mean UMUX usability score was 6.01, %(scale of 1-7), 
indicating high perceived usability, though slightly below the mean for the positive condition (6.19). Self attribution was also quite high (M  = 5.66) %on a scale of 1-7) 
indicating that users felt responsible for the outcomes of using the technology, though scores on this measure were high for most groups.

\paragraph{Free text answers}
% QUAL STUFF 
%When participants in this category discussed qualities of the technology, they more often 
The majority of participants in this profile discussed positive qualities of the technology (64\%), often focusing on convenience and ways the technology made things easier.
% A few indicated that the technology was exceptional in some way: better than equivalent options or continually improving. 
More than in any other profile, users described how the technology was well adapted to their needs and tastes, and able to integrate into their wider routine (19\%). 
% For example:
% "It was like a blank canvas, ready to be customised to fit my unique needs. I started small [...] but soon discovered the true power of this app." [ID343]. 
Negative qualities were mentioned less often than in other groups (21\%).
% , with small numbers feeling that the technology was e.g. hard to understand (4\%), had bugs (5\%) or failed to live up to expectations (4\%).

Further, participants described more active attitudes of engagement than other groups. Around half (48\%) indicated self-driven modes of engagement, such as goal-oriented learning, career development, and pursuit of health and fitness. %Around 12\% mentioned the self-tracking of goals. 
Self-driven engagement was also evident in discussion of customising and becoming proficient in the technology, %or in participants emphasising their control or mastery of the technology, 
and technology use was often related to personal passions and interests (30\%), such as scientific research, %ID101
arts, spiritual learning, or fandom: ``i  have learned painting through ticktok  and it has now became my new hobby. I  also use it to get more insights on spiritual teachings so i can advance in  my spiritual journey.'' (ID390)
Creative and generative attitudes were more common than in other groups (19\%): creating music, text, and video, or actively seeking inspiration and new ideas. 
% Along these lines participants discussed using the technology to explore aspects of themselves, % ID390, 91, 127
% or open up perspectives on new people and places. %ID550
% More participants in this group used the technology for self-tracking of goals (12\%) than in other groups, and more related the technology to personal passions and interests (30\%), from scientific research %ID101
% to arts, spiritual learning, and sports fandom. 
Entertainment (28\%), connection to others (32\%), staying up to date (17\%), and financial goals (16\%) were all well represented. %, but not more usual for the other groups. 
Comparatively few users (8\%) mentioned using the technology to escape or relax.


Members of the High Quality profile commonly mentioned aspects of their own identity. Quite a few prefaced positive evaluations with identity statements like ``as a DJ'' (ID152), ``as a woman and as a mom'' (ID134). Others explicitly connected the technology to professional and enthusiast identities such as ``content creator'' (ID523), ``marketing manager'' (ID233), or ``gamer'' (ID640), or linked it to self expression 
% (ID214) 
or meaningful work.
% (ID101).
A small number described value-agreement with the technology: mentioning their good opinion of the tech's makers, sustainability, fairness, and other ethical values. Disagreements with values %perceived in the technology were 
was uncommon compared to other profiles.

Finally, it was more common for %participants in 
this profile to emphasise positive emotional associations with the technology: e.g., connecting the app to family meaning, good memories, or a sense of community. Compared to other profiles, participants were also more likely to connect the technology to things that were good for them: supporting health and fitness, addressing personal challenges, enacting self care, or exploring new perspectives and aspects of themselves. %ID605, 225 % ID390, 91, 127



\subsubsection{Medium}
\paragraph{Participants and Technologies}
% High level categorical stuff
This profile contains 146 participants, 111 of whom (76\%) were in the positive condition.
In general, the distribution of technologies was similar to the High Quality profile (see \autoref{tab:profile_technologies}): Social media was most common (25\%). %, and a diverse range of other technology types were represented, including creativity, messaging and computers, tablets and phones. 
Notably, in the Medium profile a larger percentage discussed streaming media technologies such as Youtube and spotify (18\% vs 8\%), whereas technologies for fitness, health and well-being were discussed less (1\% vs 8\%).


\paragraph{Motivational regulations}
This group showed a similar skew towards more autonomous motivations, though with lower values than in the High Quality group. The most prominent motivation in this profile was intrinsic motivation, followed by identified regulation. %, suggesting that motivation was in large part due to the inherent interest or fun of the technology, and the sense that using it is worthwhile. 
%Both of these scores were a little lower than in the High Quality group, but high compared to other groups. 
Integrated regulation was notably lower than in the High Quality group, indicating less deep personal investment in the technology. %, or lower congruence with values.
% --- and in fact this was also lower than in the otherwise less autonomous External group.  
Introjection, external regulation, and amotivation scores were low, with introjection notably lower than in the High Quality profile. %, and the other scores comparable. 
%This suggests that participants generally used the technology without much motivation by risk, external reward, or for example guilt, and they used it in an fairly intentional way. 

% External variables
%\paragraph{Need satisfaction}
\paragraph{UX ratings}
% External variables
Need satisfaction for this profile was moderate. %Overall satisfaction for the three basic needs (3.5) and for the full eight needs (3.22) sat just below the midpoint of the means for positive and negative conditions. 
While this profile showed the second highest mean score %of any group 
for autonomy (M  = 3.98), scores for competence (M  = 3.54) and relatedness (M  = 2.97) ranked below the External profile (see below). In contrast to the High Quality profile, self-actualising-meaning (M  = 2.40), self-esteem (M  = 3.60), and security (M  = 3.35) scores were low --- close to the negative condition means. 
% Pleasure (3.56) was close to halfway between the means for negative and positive conditions.


%\paragraph{Other Outcome Variables}
The mean PANAS score was 1.55, indicating moderately positive affect. This was the second highest affect of all groups, and slightly below the mean for the positive condition. Usability was rated relatively highly (M = 5.97). %, very close to the High Quality condition, though again slightly lower than the mean for the positive condition. The mean for 
Self-attribution was pronounced (M  = 5.29), but mostly comparable to other profiles. %While indicating a strong sense of responsibility for the outcomes of using the technology, this value is not  high in comparison to other groups in the study.



\paragraph{Free text answers}
% QUAL STUFF 
Discussion of technology qualities %in this group was very 
was similar to the High Quality profile. Most participants in this group (62\%) attributed positive qualities to the technology itself, focusing on convenience, ease, and adaptation to needs. Negative qualities such as bugs, and difficulty in use were mentioned relatively infrequently (19\%).

Purposes of technology use were again similar to %those in 
the High Quality profile. Both profiles were likely to use the technology for self-development (40\% vs 42\%), connecting with others (33\% vs 32\%), and  money goals (17\%, vs 16\%). Escapism (14\%) %vs 8\% in High Quality)
and entertainment (34\%) %vs 28\%) 
were slightly more common in this profile.
Descriptions of engagement were slightly less likely to emphasise %than in the High Quality profile to indicate a strongly 
self-driving attitudes (e.g. seeking to make a contribution, or pursuing self-organisation or fitness: 38\% vs 48\%). There was also a slightly lower emphasis on connection to personal interests and passions (25\% vs 30\%), and on creative and generative modes of engagement such as thinking, creating and self-expressing (15\% vs 19\%).
In contrast, users in this group were more likely to describe their technology use as determined by external factors e.g., chosen by their employer, or due to lack of good alternatives: 10\% vs 5\%. For example: ``I have to continue using it cause everyone else does'' (ID672).
A higher percentage also indicated that their use was marked by some degree of compulsion, overuse or empty habit (8\% vs 3\%). 
%However, despite differences, in all of these cases the Medium profile was closer to the High Quality profile than it was to the other groups, discussed below.

%There was a greater difference from the High Quality profile in how participants' discussed whether the technology was good or bad for them. 
Compared to the High Quality profile, fewer respondents indicated they felt the technology was good for them (18\% vs 27\%). 
% - a similar proportion to that found in the Amotivated IM group discussed below. 
%In particular, fewer discussed ways in which the technology supported health and fitness, or addressed personal challenges. 
Conversely, slightly more participants discussed ways in which the technology was bad for them (12\% vs 8\%), though there were no clear thematic patterns. %or distinctions 
%in how the technology was considered bad.

The largest difference from the High Quality profile concerned %how the technology related to participants 
values, identity and emotional connection. It was more common for participants in the Medium profile to emphasise that the technology had no personal meaning: serving only as entertainment or a neutral tool (18\% vs 4\%), e.g. ``they don't mean anything really, i just like them.'' (ID147). 
More also indicated some kind of value misalignment with the technology (4\% vs 10\%), focusing, for example, on %bad 
opinions of the company
and unwanted exposure to political ideology.
Slightly fewer accounts indicated emotional connection to the technology (11\% vs 14\%), or ways in which the technology connected positively to the participant's identity (12\% vs 19\%). However, both positive emotional and identitarian aspects were still considerably more common than in the remaining profiles discussed below.


\subsubsection{External}
\paragraph{Participants and Technologies}
% High level categorical stuff
This group contains 58 participants, 11 (19\%) of whom were in the positive condition.
A less diverse range of technology types was found in this group, with 60\% of the responses addressing three technology categories: Social media (21\%), workplace technologies (22\%), and messaging technologies (17\%). %Otherwise no category was chosen by more than 5\% of participants. 

\paragraph{Motivational regulations}
% UMI scores
The profile showed a strong left-skew, towards less autonomous motivations. External regulation was most prominent, %(indicating motivation via external reward and avoidance of punishment), 
followed by introjection. %(indicating rigid internal controls such as guilt, shame, or contingent self-esteem). 
Both were substantially higher than in all other groups. However, alongside these highly controlled motivations, identified and integrated regulations sat at around the same level as in the more autonomous Medium Quality group, suggesting that participants in the External profile were no less likely to perceive the outcome of the activity as personally meaningful, nor less likely to identify with the activity.
Intrinsic motivation, meanwhile, was very low in comparison to most profiles, indicating that there was relatively little pleasure or interest inherent in the use of the technology. Amotivation was high in comparison to both the High Quality and Medium groups --- suggesting that users in this group were less intentional and conscious in their engagement.


%\paragraph{Need satisfaction}
\paragraph{UX ratings}
% External variables
Overall need satisfaction was moderate, yet %means %for totals on the three basic needs (3.64) and the full 8 needs (3.32) 
%sat close to the midpoint between values for the negative and positive conditions. %In both cases these values are slightly higher than for the Medium group, making this the second most needs-satisfying of the profiles.
satisfaction for individual needs varied considerably.
Autonomy (3.26) sat below the negative condition mean. Competence (3.86) sat between negative and positive means. Relatedness (3.80) was above the positive condition mean, close to that for the High Quality profile (4.09).  %The group ranked second highest on these latter two needs, and the relatedness value sat close to that for the High Quality group (4.09). 

Turning to the additional needs: Stimulation (2.77) was particularly low --- beneath the negative condition average, and the second lowest among profiles. 
Self-actualising-meaning (2.40) and self-esteem (3.51) were also low, though close to values for the Medium Quality group. Security (3.77) and Popularity (3.24) were relatively high: higher than any group apart from High Quality, and only slightly below the respective positive condition means. 

%\paragraph{Other Outcome Variables}
Average PANAS score was 0.36, indicating neutral affect: considerably lower than both the High and Medium Quality profiles, and below the negative condition mean. Perceived usability was also low %in the context of the data-set 
(4.03), placing it comfortably below the negative condition mean.
Self-attribution (5.23) sat close to the negative condition mean.


% QUAL STUFF 
\paragraph{Free text answers}
Descriptions of the technology focused most on negative qualities. Common criticism was that the technology was difficult to use or understand (34\%), e.g., ``For me this programme is really hard to master'' (ID518). %- higher than any other category), %but participants also emphasised 
It was also common to note markers of low quality such as bugs, weak content, and poor comparison to competitors (22\%), and a range of other problems (19\%).
Positive evaluations were less common (22 \%) and focused largely on ways in which the technology was user-friendly, saved time or made something easier (14\%). 
% It was rare for participants in this group to indicate the technology was well adapted to them and their needs (3\%).

The most common purposes mentioned by participants was work (40\%) %--- reflecting the commonness of workplace technologies in this group. 
%It was also common for participants to emphasise 
and connecting with others (40\%). Both purposes were more strongly represented than in other groups. Purposes of self-development (16\%) were %lower, and 
far less common than in the High and Medium Quality profiles, as were strongly self-driven attitudes of engagement (24\% - lower than any but Amo IM). 
Notably, more than half of participants in this group indicated that their use of the technology was determined by factors beyond their control (55\% - far higher than other categories) such as a requirement of their employer, or occasionally their school. 
Passive engagement was relatively uncommon: less participants mentioned escaping and relaxing than in any other category (2\%), and relatively few indicated compulsive or habitual use (10\%).

Compared to other profiles, few participants %in the External group 
indicated that the technology was good for them (5\%). Meanwhile, 24\% indicated that the technology was bad for them: high compared to the High (8\%) and Medium Quality (12\%) groups, but low compared to the Amotivated (35\%) and Amo-IM groups (61\%), discussed below. %The technology could be bad for the user in quite diverse ways but more 
Common individual factors concerned impact on self-image (e.g. comparing oneself to others, or feeling incompetent), and risk of privacy violation. 
While not all accounts in this group were so negative, an excerpt from participant ID350 captures many of the issues common in this profile \textit{``Despite feeling like the app is harmful to  my mental health, I keep using it because I feel like it might be helpful. I  might land a dream job or connect with someone who can help me excel in my  career. In some ways, it's also to torture myself and compare myself to  others (gives me something to work towards, in an odd way).''}


\subsubsection{Amotivated - Intrinsic}

\paragraph{Participants and Technologies}
% High level categorical stuff
This group contains 71 participants, only 7 of whom (9.9\%) were in the positive condition.
The technology types in this category were quite homogeneous: 73\% wrote about social media, 17\% about entertainment categories (streaming media (7\%), gaming (6\%), other entertainment (4\%). %No other category was selected by more than two participants.

 \paragraph{Motivational regulations}
The motivations in this profile had a scooped structure (see \autoref{lpa_profiles}). Amotivation was the most prominent regulation, and higher than in any other profile, while none of the other regulations were especially high. Together this indicates a relative lack of intentionality, and relatively little conscious valuing of the activity. Identified regulation, and introjection scores was lower than any other group, indicating that users did not value the outcomes and consequences of interaction, but nor were they motivated by internalised shame or contingent self esteem. Internalised regulation scores were also low: indicating little personal identification with the activity. 

Within this relatively low motivation context, however, intrinsic motivation was relatively high --- only a little lower than in the %quite autonomous 
Medium Quality profile. This suggests that pleasure and interest inherent in the activity itself were the primary \emph{conscious} motivators. External motivation scored a little lower, %(comparable to the High Quality group) 
indicating some role for external rewards or the avoidance of punishment. 



%\paragraph{Need satisfaction}
\paragraph{UX ratings}
% External variables
Overall need satisfaction for this profile was low. %Satisfaction for both the three basic needs (2.62) and for the full 8 needs (2.68) both sat below the negative condition means, and this was the second least satisfied group overall. 
Individual need satisfaction scores averaged below the negative condition mean in all but one case: Pleasure (3.48) sat between the negative and positive condition means, close to the value for the Medium Quality group (3.56).
Of the three basic needs, autonomy (3.07) and relatedness (2.72) were slightly below their respective negative condition means, while competence (2.08) was considerably lower than any other profile. 


%\paragraph{Other Outcome Variables}
Mean PANAS score was 0.21, indicating neutral affect --- close to the score for the External profile, and slightly below the negative condition mean. 
Perceived usability (5.52) and %was relatively high, and not so far below the High Quality (6.01) and Medium (5.97) groups.
%This group also had the second highest 
self-attribution (5.57) scored relatively high.


\paragraph{Free text answers}

Compared to other profiles, respondents %these users 
gave little attention to the qualities of the technology itself. %: e.g. to how good the tech was at its job, bugs and errors, functioning, how hard it was to use, the quality of the content. Only \sim30\% of participants addressed these issues, compared to roughly 70-88\% in other groups. Most of these participants 
Most discussed negative qualities (28\%), often focusing on the behaviour of others technology users (bad moderation, lies, and misinformation discussed in $\sim15\%$ of responses), and the perception that behaviour on the service had declined ($\sim14\%$). %For example (ID398) ``I feel like Tik Tok has taken a turn, where people keep posting only negative videos in order to gain likes and views.''. 
The few mentions of positive qualities ($\sim8\%$) such as convenience were often expressed in unenthusiastic terms (e.g. ID434  `` they don't necessarily mean that much to me [...] I just bought them for convenience'').

When discussing the purpose of the technology, participants tended to emphasise entertainment (49\%), and escapism (30\%): in both cases much more commonly than in other groups. %( 34\% and 14\% for the next highest group in each case). 
25\% (more than other groups) mentioned using the technology to stay informed on current affairs, entertainment news and trends. 
Some accounts indicated a role for the app in self-development (20\%): mostly concerning access to life-hacks, fitness tips, and motivational materials. %that ``inspire me do work hard on myself''(ID166 sic), 
However, such mentions were often unspecific, and functioned to hedge wider criticism (e.g. ``You  discover and learn many new things that improve your life. But you waste a lot of time in the app and you compare yourself a lot with other people'': ID111).
As in most other groups, it was common to mention using the technology to connect with other people, or keep up to date with their lives (28\%.)

The attitude of engagement in this group was far more passive than in other profiles: 63\% (three times the next-ranked group) mentioned wasting time, habitual use, or reactive engagement such as FOMO, and following clickbait. Only 8\% %(vs 24\% for the next lowest group) 
described self-driving behaviours. %: often focusing on fitness, career and personal learning goals. 
Less active engagement like lurking and consuming media was far more common (32\%), as were escaping and relaxing (32\%). 
% The most active engagement in this group concerned active sharing of media and personal ideas, actively following topics of interest, and efforts to engage mindfully with the technology. These styles of engagement were coded at roughly the same level, or slightly higher than in other groups.
%However, despite the relatively passive character of their engagement, fewer users in this group than in others indicated that the tech was chosen or imposed by others. 


Participants %in this group 
commonly discussed ways in which they felt the technology was bad for them ($\sim60\%$). %vs 35\% or less in all other groups). 
Mostly this centred on the feeling that their use of the technology was compulsive (41\%), and several indicated that they felt addicted. 
Compared to other groups, it was very common for users to feel that the technology diminished their emotional state or well-being, diminishing their self-image, or damaging mood (31\%). %vs 18\% or less in other groups). Users 
Respondents also felt that the technology degraded %behaviours and capacities: damaging 
their attention span and brought out negative personal traits (14\%). %vs 7\% or less). 
% Users in this group were often highly conflicted about the technology: most strikingly in one participant who described his own toxic behaviour in the game League of Legend, tied to a difficult period in his life, while simultaneously emphasising memories and meaningful friendships.

% Compared to other groups, users in this group discussed the relation of the technology to values, identity and emotional connection (75\% of participants, vs 55\% or less in other groups): though largely in negative terms. 
Compared to the other profiles, it was also more common to express disagreement with the values embodied by the technology (38\%). Often this focused on the participant's poor view of the community of users, %: their ``fake'' presentation, and their offensive views. participants also discussed 
or disagreement with the company behind the technology. %: via bias, bad behaviour and over-commercialisation. 
Outside this, participants commonly felt that the technology did not relate significantly to their values and goals (31\%). Many emphasised that the technology was merely for entertainment or distraction: ``it means nothing, I only use to distract my mind'' (ID164), ``At this moment it means nothing except a technology I have to stop using'' (ID521).



\subsubsection{Amotivated}
\paragraph{Participants and Technologies}
% High level categorical stuff
Of 57 participants in this profile only 2 (3.5\%) were in the positive condition.
%Technology types in this category were diverse: 
Most participants (23\%) wrote about social media. Other technologies, included shopping apps ( 9\%), voice assistants (9\%), and tools for creativity, media and writing (7\%). %No other category in the remaining $\sim50\%$ was chosen by more than 5\% of participants.


\paragraph{Motivational regulations}
% UMI scores
Amotivation was the highest scoring regulation for this profile, though lower than in the Amotivated-Intrinsic group. All other regulations were low relative to other groups, suggesting low overall intentionality and motivation to use the technology.
Controlled (i.e., external and introjected) regulations scored highest. Scores for integrated and intrinsic regulations were lower than in any other group, and identified regulation was similarly low, but a little higher than in the Amotivated-Intrinsic profile.


%\paragraph{Needs Satisfaction}
\paragraph{UX ratings}
% External variables
%Total need satisfaction --- both for the three basic needs (2.32) and for the full 8 needs (2.09) --- was lower than in any other group. 
Except in one case, individual need satisfaction scores were low compared to all other profile, and low in absolute terms (below 2.5). The exception was competence (2.79), which was %substantially 
higher than in the Amotivated-Intrinsic group, but still lower than all other profiles.

%\paragraph{Other Outcome Variables}
A mean PANAS score of -0.14 indicated neutral affect, but less positive than any other group. Mean usability was  at 3.15, lowest among all profiles, %--- the only group mean which fell below the halfway point of the scale UMUX, 
indicating notably greater usability issues in this condition than elsewhere.
While mean self-attribution mean was above midpoint (4.23), this profile exhibited the lowest score overall, even when compared to the negative condition (M = 5.13). %notably low within the context of the data-set, indicating that these users felt less responsibility for outcomes than users in other groups. 


\paragraph{Free text answers}
In contrast to the Amotivated-Intrinsic group,descriptions of the Amotivated profile often focused on the qualities of the technology (88\%). Negative evaluations of the technology (75\%), and in particular expressions of disappointment (30\%) were strongly represented.  %than in other groups. 
Participants often emphasised the decline of the technology (e.g. ``It was a good app at the  begenning [sic] but now it is a trash.''  ID396) or its failure to live up to expectations. It was also common to discuss low quality in software and content (35\%), the difficulty of the technology (25\%) and inconveniences like frustrating interfaces and slow functioning (26\%). Notably, positive evaluations of the technology were not uncommon %, reported by a higher percentage of users than in either the External or Amotivated-Intrinsic groups 
(30\%). Mostly, however these positive evaluations were often emphasised as being in conflict with wider problems. One participant, for instance, enjoyed the convenience of face-recognition but felt discomfort at the idea of losing anonymity (ID237). Another was concerned by the effectiveness of a technology for helping their child sleep, fearing the child would become reliant (ID483).

%A large number of 
It was common for users in this group to indicate that they engaged with the technology for reasons beyond their control (30\%), %- higher than any group except External), 
and a larger proportion than in any other group indicated some intention to quit using the technology (9\%). %Creative and generative styles of engagement with the technologies were uncommon (5\%), as was the active sharing and consuming of media and content (7\%), and a
Among the social media users in the group, many described ``lurking'' behaviour: reading but not posting (7\%: higher than any other profile).
Despite this, and despite the high score for amotivation, some users in the group described engaging in quite active ways: %A relatively large number described u
Using the technology in self-driving ways (25\%), mostly by indicating active use for business or career development, money management or money-making. This was similar to the External group, and far higher than the Amotivated-Intrinsic group. %Few indicated that they used the technology to escape or relax (5\%).
%The purposes of use in this profile were quite diverse: 
Pursuit of money goals %(managing or making money) 
was more common in this profile than others (21\%), while purposes were rarely connected to personal passions and interests (4\%). Compared to other profiles, participants were also less likely to use the technology to connect with others (14\%), pursue self-development (16\%), or entertainment (21\%). 

Participants in the Amotivated profile rarely indicated that they felt the technology was good for them (7\%), while 35\% felt it was bad for them: high compared to all except the Amotivated-Intrinsic group (68\%). More often than in other groups, participants mentioned compulsion and addiction (11\%) and negative impacts on emotional state and wellbeing (18\% e.g. ``There's  good useful and interesting stuff on Instagram, but it's always the stuff  that makes me feel bad about myself that I spend more time getting sucked  into, rather than the good.'' ID205). 

Finally, more than in other profile, participants emphasised that the technology lacked personal meaning or value (33\%).
Similarly, %Compared to other groups, 
these participants rarely discussed the technology in relationship to their identities (4\%), or indicated positive emotional associations (2\%)
As in the Amotivated-Intrinsic group, users often thought that the technology disagreed with their values (23\%), often due to a bad view of the company behind the technology, or frustration with exposure to unwanted content: e.g. `` It represents the aggresive capitalism around me which goes against my values.'' (ID295).




% The fewest significant comparisons were found for Self-Attribution: comparisons between the Amotivated group and all others were significant, as was the comparison between High Quality and Medium.




\db{END OF OLD MOTIVATIONAL PROFILES COMPARISON}
